TFix+: Self-configuring Hybrid Timeout Bug Fixing for Cloud Systems

Timeout bugs can cause serious availability and performance issues which are often difficult to fix due to the lack of diagnostic information. Previous work proposed solutions for fixing specific type of timeout-related performance bugs. In this paper, we present TFix+, a self-configuring timeout bug fixing framework for automatically correcting two major kinds of timeout bugs (i.e., misused timeout bugs and missing timeout bugs) with dynamic timeout value predictions. TFix+ provides two new hybrid schemes for fixing misused and missing timeout bugs, respectively. TFix+ further provides prediction-driven timeout variable configuration based on runtime function tracing. We have implemented a prototype of TFix+ and conducted experiments on 16 real world timeout bugs. Our experimental results show that TFix+ can effectively fix 15 out of tested 16 timeout bugs.

==> Makefile <==
myfile=main
all: 
	latex $(myfile)
	bibtex $(myfile)
	latex $(myfile)
	latex $(myfile)
	dvips -o $(myfile).ps $(myfile).dvi
	ps2pdf $(myfile).ps $(myfile).pdf
pdf:
	latex $(myfile)
	latex $(myfile)
	dvips -o $(myfile).ps $(myfile).dvi
	ps2pdf $(myfile).ps $(myfile).pdf

clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc *.dvi $(myfile).dvi\
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd *.bak *.tex.bak\
	*.dvi *.ps *.thm *.tgz *.zip *.rpi *.pdf
        


==> acknowledgments.tex <==

We would like to thank the anonymous reviewers for their valuable comments. This research is supported in part by NSF CNS1513942 grant and NSF CNS1149445 grant. Any opinions expressed in this paper are those of the authors and do not necessarily reflect the views of NSF.


==> affectedFuns.tex <==
\begin{table}[!t]
\centering
\caption{The timeout affected functions.}
\label{affected_result}
\scriptsize
\begin{tabular}{|c|c|}
\hline
\textbf{Bug ID}       & \textbf{Timeout Affected Functions} \\ \hline\hline
Hadoop-9106           &  Client.setupConnection()          \\ \hline
Hadoop-11252 (v2.6.4) &  RPC.getProtocolProxy()        \\ \hline
Hadoop-10695 &  KMSClientProvider.creatConnection()       \\ \hline
HDFS-4301             &  TransferImage.doGetUrl()         \\ \hline
HDFS-10223            &  \begin{tabular}[c]{@{}c@{}}DFSUtilClient \\ .peerFromSocketAndKey()\end{tabular}         \\ \hline
HDFS-9887            & \begin{tabular}[c]{@{}c@{}} URLConnectionFactory \\ .openConnection()\end{tabular}         \\ \hline
MapReduce-6263        &  YARNRunner.killJob()         \\ \hline
MapReduce-4089        &  \begin{tabular}[c]{@{}c@{}}TaskHeartbeatHandler \\ .PingChecker.run() \end{tabular}       \\ \hline
Yarn-1630 (v2.3.0) &   YarnClientImpl.submitApplication()      \\ \hline
HBase-15645           &  RpcRetryingCaller.callWithRetries()         \\ \hline
HBase-17341           &  ReplicationSource.terminate()          \\ \hline                                                                                                                                          
\end{tabular}
\end{table}

==> differentiate.tex <==
\begin{table*}[!t]
\centering
\caption{TFix's classification result of timeout bugs.}
\label{fe_match}
\scriptsize
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Bug ID}       &  \textbf{Bug Type}  & \textbf{Matched Timeout Related Functions}                                                                                                                                               & \textbf{\begin{tabular}[c]{@{}c@{}}Correct Timeout \\ Bug Classification?\end{tabular}} \\ \hline\hline
Hadoop-9106           &    too large timeout   &  \begin{tabular}[c]{@{}c@{}}System.nanoTime, URL.\textless{}init\textgreater{}, \\ DecimalFormatSymbols.getInstance, \\ ManagementFactory.getThreadMXBean\end{tabular}                                                                                                                                                                       & Yes                                         \\ \hline
Hadoop-11252 (v2.6.4) &    too large timeout  & \begin{tabular}[c]{@{}c@{}}Calendar.\textless{}init\textgreater{}, Calendar.getInstance, \\ ServerSocketChannel.open\end{tabular} &        Yes                                 \\ \hline
Hadoop-10695 &   too small timeout  &  \begin{tabular}[c]{@{}c@{}}ConcurrentHashMap.addCount, ConcurrentHashMap.putVal, \\ ConcurrentHashMap.putIfAbsent, \\ ClassLoader.getClassLoadingLock, TimeZone.getTimeZone, \\ TimeZone.setDefaultZone, TimeZone.getDefaultRef, \\ TimeZone.getDefault\end{tabular} &  Yes                                         \\ \hline
HDFS-4301             &    too small timeout  & \begin{tabular}[c]{@{}c@{}}AtomicReferenceArray.get, ThreadPoolExecutor  \end{tabular}                                                                                                                                                                 &     Yes                                    \\ \hline
HDFS-10223            &    too large timeout & GregorianCalendar.\textless{}init\textgreater{}, ByteBuffer.allocateDirect                                                                           &                   Yes                       \\ \hline
HDFS-9887          &   too small timeout  &  \begin{tabular}[c]{@{}c@{}}TimeZone.getTimeZone, TimeZone.setDefaultZone, \\TimeZone.getDefaultRef, TimeZone.getDefault, URL.\textless{}init\textgreater{} \end{tabular}                                     &        Yes                                \\ \hline
MapReduce-6263        &    too small timeout &   \begin{tabular}[c]{@{}c@{}}DecimalFormatSymbols.initialize, ReentrantLock.unlock, \\ AbstractQueuedSynchronizer, \\ConcurrentHashMap.PutIfAbsent, ByteBuffer.allocate \end{tabular}                                                                                                                                                                    & Yes                                         \\ \hline
MapReduce-4089        &    too large timeout &   \begin{tabular}[c]{@{}c@{}}charset.CoderResult, AtomicMarkableReference, \\ DateFormatSymbols.initializeData \end{tabular}                                                                                                                                                                    & Yes                                         \\ \hline
Yarn-1630 (v2.3.0)        &  too large timeout  &     \begin{tabular}[c]{@{}c@{}}  URL.isBuiltinStreamHandler, URL.\textless{}init\textgreater{}, \\ Calendar.createCalendar, Calendar.getInstance, \\ SimpleDataFormat.initializeCalendar, SimpleDataFormat.\textless{}init\textgreater{} \end{tabular}        & Yes                                          \\ \hline
HBase-15645           &   too large timeout  &   \begin{tabular}[c]{@{}c@{}}  CopyOnWriteArrayList.iterator, URL.\textless{}init\textgreater{}, \\ System.nanoTime, AtomicReferenceArray.set, \\ ReentrantLock.unlock, AbstractQueuedSynchronizer, \\ DecimalFormat.format   \end{tabular}                                                                                                                                                          &          Yes                               \\ \hline
HBase-17341           &   too large timeout  &  \begin{tabular}[c]{@{}c@{}} ScheduledThreadPoolExecutor.\textless{}init\textgreater{}, \\ DecimalFormatSymbols.initialize, System.nanoTime, \\ ConcurrentHashMap.computeIfAbsent \end{tabular}                                                                                                                                                                     &     Yes                                    \\ \hline \hline
\red{HDFS-3180}        &   Missing timeout &          None                                                                                                                                                               &          Yes                               \\ \hline
%\red{HDFS-3166}        &   Missing timeout &                                                                                                                                                                         &                                         \\ \hline
\red{HDFS-4176}        &   Missing timeout &        None                                                                                                                                                                 &               Yes                          \\ \hline
%\red{HDFS-7005}        &   Missing timeout &                                                                                                                                                                         &                                         \\ \hline
\red{MapReduce-5066}        &   Missing timeout & None                                                                                                                                                                        &      Yes                                   \\ \hline
\red{Yarn-1630 (v2.2.0)}        &  Missing timeout  &    None    & Yes                                          \\ \hline
\end{tabular}
\end{table*}

\begin{comment}
\begin{table*}[!t]
\centering
\caption{TFix's classification result of timeout bugs.}
\label{fe_match}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Bug ID}       &  \textbf{Bug Type}  & \textbf{Matched Timeout Related Functions}                                                                                                                                               & \textbf{\begin{tabular}[c]{@{}c@{}}Correct Timeout \\ Bug Classification?\end{tabular}} \\ \hline\hline
Hadoop-9106           &   \begin{tabular}[c]{@{}c@{}}Misused \\ too large timeout\end{tabular}   &  \begin{tabular}[c]{@{}c@{}}System.nanoTime, URL.\textless{}init\textgreater{}, \\ DecimalFormatSymbols.getInstance, \\ ManagementFactory.getThreadMXBean\end{tabular}                                                                                                                                                                       & Yes                                         \\ \hline
Hadoop-11252 (v2.6.4) &   \begin{tabular}[c]{@{}c@{}}Misused \\ too large timeout\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Calendar.\textless{}init\textgreater{}, Calendar.getInstance, \\ ServerSocketChannel.open\end{tabular} &        Yes                                 \\ \hline
\textcolor{red}{Hadoop-10695} &  \begin{tabular}[c]{@{}c@{}}Misused \\ too small timeout\end{tabular}  &  \begin{tabular}[c]{@{}c@{}}ConcurrentHashMap.addCount, ConcurrentHashMap.putVal, \\ ConcurrentHashMap.putIfAbsent, \\ ClassLoader.getClassLoadingLock, TimeZone.getTimeZone, \\ TimeZone.setDefaultZone, TimeZone.getDefaultRef, \\ TimeZone.getDefault\end{tabular} &  Yes                                         \\ \hline
HDFS-4301             &   \begin{tabular}[c]{@{}c@{}}Misused \\ too small timeout\end{tabular}  & \begin{tabular}[c]{@{}c@{}}AtomicReferenceArray.get, ThreadPoolExecutor  \end{tabular}                                                                                                                                                                 &     Yes                                    \\ \hline
HDFS-10223            &   \begin{tabular}[c]{@{}c@{}}Misused  \\ too large timeout\end{tabular} & GregorianCalendar.\textless{}init\textgreater{}, ByteBuffer.allocateDirect                                                                           &                   Yes                       \\ \hline
\textcolor{red}{HDFS-9887}          &  \begin{tabular}[c]{@{}c@{}}Misused  \\ too small timeout\end{tabular}  &  \begin{tabular}[c]{@{}c@{}}TimeZone.getTimeZone, TimeZone.setDefaultZone, \\TimeZone.getDefaultRef, TimeZone.getDefault, URL.\textless{}init\textgreater{} \end{tabular}                                     &        Yes                                \\ \hline
MapReduce-6263        &   \begin{tabular}[c]{@{}c@{}}Misused  \\ too small timeout\end{tabular} &   \begin{tabular}[c]{@{}c@{}}DecimalFormatSymbols.initialize, ReentrantLock.unlock, \\ AbstractQueuedSynchronizer, \\ConcurrentHashMap.PutIfAbsent, ByteBuffer.allocate \end{tabular}                                                                                                                                                                    & Yes                                         \\ \hline
MapReduce-4089        &   \begin{tabular}[c]{@{}c@{}}Misused  \\ too large timeout\end{tabular} &   \begin{tabular}[c]{@{}c@{}}charset.CoderResult, AtomicMarkableReference, \\ DateFormatSymbols.initializeData \end{tabular}                                                                                                                                                                    & Yes                                         \\ \hline
\textcolor{red}{Yarn-1630}        & \begin{tabular}[c]{@{}c@{}}Misused  \\ too large timeout\end{tabular}  &     \begin{tabular}[c]{@{}c@{}}  URL.isBuiltinStreamHandler, URL.\textless{}init\textgreater{}, \\ Calendar.createCalendar, Calendar.getInstance, \\ SimpleDataFormat.initializeCalendar, SimpleDataFormat.\textless{}init\textgreater{} \end{tabular}        & Yes                                          \\ \hline
HBase-15645           &   \begin{tabular}[c]{@{}c@{}}Misused  \\too large timeout\end{tabular}  &   \begin{tabular}[c]{@{}c@{}}  CopyOnWriteArrayList.iterator, URL.\textless{}init\textgreater{}, \\ System.nanoTime, AtomicReferenceArray.set, \\ ReentrantLock.unlock, AbstractQueuedSynchronizer, \\ DecimalFormat.format   \end{tabular}                                                                                                                                                          &          Yes                               \\ \hline
HBase-17341           &   \begin{tabular}[c]{@{}c@{}}Misused  \\too large timeout\end{tabular}  &  \begin{tabular}[c]{@{}c@{}} ScheduledThreadPoolExecutor.\textless{}init\textgreater{}, \\ DecimalFormatSymbols.initialize, \\ System.nanoTime, \\ ConcurrentHashMap.computeIfAbsent \end{tabular}                                                                                                                                                                     &     Yes                                    \\ \hline \hline
Hadoop-11252 (v2.5.0) &   Missing & None                                                                                                                                                                      &     Yes                                    \\ \hline
HDFS-1490             &   Missing & None                                                                                                                                                                        &     Yes                                    \\ \hline
MapReduce-5066        &   Missing  & None                                                                                                                                                                        &      Yes                                   \\ \hline
Flume-1316            &   Missing & None                                                                                                                                                                      &        Yes                                 \\ \hline
Flume-1819            &   Missing & None                                                                                                                                                                     &         Yes                                \\ \hline
\end{tabular}
\end{table*}
\end{comment}





==> figures/HDFS-10223.tex <==
	\begin{figure}[!t]
	\centering
	% \begin{subfigure}[b]{\linewidth}
	\begin{lstlisting}[escapechar=|, frame=single, style=baseJava, tabsize=1]					  
//TcpPeerServer.java              HDFS-10223(v2.7.0)
		@RED@+@RED@ private Configuration conf = new Configuration();
		@RED@+@RED@ private String @BG@PEERSEND_TIMEOUT_KEY@BG@ = "peersend.timeout";
		@RED@+@RED@ private int @BG@DEFAULT_PEERSEND_TIMEOUT@BG@ = 60 * 1000;
		@RED@+@RED@ private int (*@\tikzmark{c2Left}{}@*)@BG@timeout@BG@(*@\tikzmark{c2Right}{}@*) = conf.getInt(	
		@RED@+@RED@		PEERSEND_TIMEOUT_KEY, DEFAULT_PEERSEND_TIMEOUT);
		
(*@\tikzmark{bLeft}{}@*)81(*@\tikzmark{bRight}{}@*)  public static Peer peerFromSocketAndKey(...) throws IOException {
		@RED@+@RED@		@BG@peer.setReadTimeout(timeout);@BG@//provided API
(*@\tikzmark{cLeft}{}@*)90(*@\tikzmark{cRight}{}@*)   peer = saslClient.peerSend(peer, ...);
						...
98  }    
\end{lstlisting}
% \begin{tikzpicture}[overlay,remember picture]
% 				\renewcommand{\VerticalShiftForOverLArrows}{0.0em,1ex}
% 				\renewcommand{\VerticalShiftForBelowRArrows}{0.0em,0.0ex}
% 				\renewcommand{\VerticalShiftForArrows}{0.0em,0.0ex}
% 				\renewcommand{\VerticalShiftForArrowsRtoLEnd}{-3.2em,2.4ex}
% 				\renewcommand{\VerticalShiftForArrowsRtoRStart}{3.2em,2.0ex}
% 				% \DrawArrowsRtoR[gray, in=0, out=-63]{b1}{a1}
% 				% \DrawArrowsRtoR[gray, in=63, out=-63]{c1}{b1}
% 				% \DrawArrowsLtoL[azure, in=130, out = -120, solid]{a}{b}
% 				% \DrawArrowsOverLtoBelowR[gray]{d2}{b2}
% 				% \DrawArrowsOverLtoBelowR[gray]{a1}{c2}
% 				% \DrawArrowsRtoR[gray, in=-50, out=55]{e2}{a2}
% \end{tikzpicture}
% \end{subfigure}
% \vspace*{-1.7\baselineskip}
\caption{
Code snippet of HDFS-10223 bug. 
Without setting timeout for network connection, the {\tt TcpPeerServer} hangs on reading from an unresponsive DataNode.
%To save space, we omit the call paths: {\tt newConnectedPeer()} $\rightarrow$ {\tt peerSend()} $\rightarrow$ {\tt checkTrustAndSend()}
%$\rightarrow$ {\tt send()} $\rightarrow$ {\tt getEncryptedStreams()} $\rightarrow$ {\tt doSaslHandshake()} $\rightarrow$ {\tt readSaslMessage()} $\rightarrow$ {\tt vintPrefixed} $\rightarrow$ {\tt read()}.
% ``{\color{red}-}'' means deleted code and 
``{\color{red}+}'' means added code, representing the patch generated by TFix.
% ``{\protect\bluearrowsolid}'' represents the function call flows.
% ``{\protect\grayarrowdenselydotted}'' represents the data dependency flow.
}
\label{fig:HDFS-10223}
\end{figure}


==> figures/HDFS-4301.tex <==
\begin{figure}[!t]
\centering
\begin{small}
\hfill
\begin{minipage}{.465\textwidth}
\begin{lstlisting}[frame=single, style=baseJava]
//SecondaryNameNode class
360 public void doWork() {
     ...
368  while (shouldRun) {
      ...
377   try {
       ...
(*@\tikzmark{aLeft}{}@*)386(*@\tikzmark{aRight}{}@*)    doCheckpoint();
       ...
(*@\tikzmark{g1Left}{}@*)389   } catch (IOException e) {(*@\tikzmark{g1Right}{}@*)
390    LOG.error("Exception ...");
       ...//simply logged and then retry
404  }
405 }

(*@\tikzmark{bLeft}{}@*)504(*@\tikzmark{bRight}{}@*) public boolean doCheckpoint() throws (*@\tikzmark{f1Left}{}@*)IOException(*@\tikzmark{f1Right}{}@*) {
     ...
(*@\tikzmark{cLeft}{}@*)558(*@\tikzmark{cRight}{}@*)  TransferFsImage.uploadImageFromStorage(...);
     ...  
568 }

//TransferFsImage class
(*@\tikzmark{dLeft}{}@*)168(*@\tikzmark{dRight}{}@*) public static void uploadImageFromStorage(...) 
169                             throws (*@\tikzmark{e1Left}{}@*)IOException(*@\tikzmark{e1Right}{}@*) {
     ...
(*@\tikzmark{eLeft}{}@*)176(*@\tikzmark{eRight}{}@*)  TransferFsImage.getFileClient(...);
     ...
191 }

(*@\tikzmark{fLeft}{}@*)250(*@\tikzmark{fRight}{}@*) static ... getFileClient(...) throws (*@\tikzmark{d1Left}{}@*)IOException(*@\tikzmark{d1Right}{}@*) {
     ...                  //HTTP GET request
254  URL url = new URL(..."/getimage?"...);
(*@\tikzmark{gLeft}{}@*)255(*@\tikzmark{gRight}{}@*)  return doGetUrl(url, ...);
256 } 

(*@\tikzmark{hLeft}{}@*)258(*@\tikzmark{hRight}{}@*) public static...doGetUrl(...) throws (*@\tikzmark{c1Left}{}@*)IOException(*@\tikzmark{c1Right}{}@*) {
     ...
261  HttpURLConnection connection;
     ...            /*too small timeout value*/
277  connection.setReadTimeout(@RED@timeout@RED@);
     ... 
319  InputStream stream = connection.getInputStream();
     ...
(*@\tikzmark{a1Left}{}@*)358  num = stream.read(buf);(*@\tikzmark{a1Right}{}@*)
     ... 
401 }                                    (*@\tikzmark{b1Left}{}@*)(*@\tikz[overlay,right]\node[mynode,fill=white,yshift=-1ex]{\makecell{Throw\\ Exception}};@*)(*@\tikzmark{b1Right}{}@*)

\end{lstlisting}
\end{minipage}
\hfill
\begin{tikzpicture}[overlay,remember picture]
    \renewcommand{\VerticalShiftForArrows}{0.0em,0.0ex}
    \renewcommand{\VerticalShiftForArrowsRtoLEnd}{-3.2em,2.4ex}
    \renewcommand{\VerticalShiftForArrowsRtoRStart}{3.2em,2.0ex}
    \DrawArrowsLtoL[azure, in=110, out = -120, dashdotted]{a}{b}
    \DrawArrowsLtoL[azure, in=120, out = -160, dashdotted]{c}{d}
    \DrawArrowsLtoL[azure, in=120, out = -160, dashdotted]{e}{f}
    \DrawArrowsLtoL[azure, in=120, out = -160, dashdotted]{g}{h}
    \DrawArrowsRtoL[gray, in=165,out=-15]{a1}{b1}
    \DrawArrowsRtoR[gray, in=-65,out=25]{b1}{c1}
    \DrawOverBelowArrows[gray]{c1}{d1}
    \DrawOverBelowArrows[gray]{d1}{e1}
    \DrawOverBelowArrows[gray]{e1}{f1}
    \DrawOverRightArrows[gray, in=-10,out=110]{f1}{g1}
    % \DrawBelowOverArrows[gray]{a}{b}
    % \DrawBelowOverArrows[gray]{c}{d}
%    \DrawArrowsRight[azure, in=-10, out = 50, dashdotted]{f1}{f2}
\end{tikzpicture}

\caption{The code snippet of the HDFS-4301 Bug.
The {\protect\bluearrowdashdotted} represents the function call flows,
while the {\protect\grayarrowdenselydotted} represents how {\tt IOException} happens and how it is thrown, catched and handled by the Secondary NameNode.
% The {\protect\grayarrowdenselydotted} represents how the {\tt Balancer} makes the configurable timeout changed from 1 min to 20 mins. 
}
\vspace*{-0.1\baselineskip}
\label{fig:HDFS-4301}
\end{small}
\end{figure}

==> figures/Mapreduce-5066.tex <==
	\begin{figure}[!t]
	\centering
	% \begin{subfigure}[b]{\linewidth}
	\begin{lstlisting}[escapechar=|, frame=single, style=baseJava, tabsize=1]					  
//JobEndNotifier.java        MapReduce-5066(v2.0.3-alpha)
		@RED@+@RED@ private Configuration conf = new Configuration();
		@RED@+@RED@ private String @BG@NOTIFICATION_TIMEOUT_KEY@BG@ = "notification.timeout";
		@RED@+@RED@ private int (*@\tikzmark{c2Left}{}@*)@BG@timeout@BG@(*@\tikzmark{c2Right}{}@*) = conf.getInt(	
		@RED@+@RED@				NOTIFICATION_TIMEOUT_KEY);
		
(*@\tikzmark{bLeft}{}@*)133(*@\tikzmark{bRight}{}@*)  private static int httpNotification(...) throws IOException {
						...
(*@\tikzmark{cLeft}{}@*)135(*@\tikzmark{cRight}{}@*)   HttpClient m_client = new HttpClient();
		//pre-configured timeout mechanisms
		@RED@+@RED@		@BG@m_client.getParams().setSoTimeout(timeout);@BG@
		@RED@+@RED@		@BG@m_client.getParams().@BG@
		@RED@+@RED@							@BG@setConnectionManagerTimeout(timeout);@BG@
						...		
(*@\tikzmark{cLeft}{}@*)138(*@\tikzmark{cRight}{}@*)   return m_client.executeMethod(method);
139  }    
\end{lstlisting}
% \begin{tikzpicture}[overlay,remember picture]
% 				\renewcommand{\VerticalShiftForOverLArrows}{0.0em,1ex}
% 				\renewcommand{\VerticalShiftForBelowRArrows}{0.0em,0.0ex}
% 				\renewcommand{\VerticalShiftForArrows}{0.0em,0.0ex}
% 				\renewcommand{\VerticalShiftForArrowsRtoLEnd}{-3.2em,2.4ex}
% 				\renewcommand{\VerticalShiftForArrowsRtoRStart}{3.2em,2.0ex}
% 				% \DrawArrowsRtoR[gray, in=0, out=-63]{b1}{a1}
% 				% \DrawArrowsRtoR[gray, in=63, out=-63]{c1}{b1}
% 				% \DrawArrowsLtoL[azure, in=130, out = -120, solid]{a}{b}
% 				% \DrawArrowsOverLtoBelowR[gray]{d2}{b2}
% 				% \DrawArrowsOverLtoBelowR[gray]{a1}{c2}
% 				% \DrawArrowsRtoR[gray, in=-50, out=55]{e2}{a2}
% \end{tikzpicture}
% \end{subfigure}
% \vspace*{-1.7\baselineskip}
\caption{
Code snippet of MapReduce-5066 bug. 
Without setting timeout for HTTP connection, the {\tt JobEndNotifier} hangs on {\tt HttpClient.executeMethod()} on line 138.
%To save space, we omit the call paths: {\tt newConnectedPeer()} $\rightarrow$ {\tt peerSend()} $\rightarrow$ {\tt checkTrustAndSend()}
%$\rightarrow$ {\tt send()} $\rightarrow$ {\tt getEncryptedStreams()} $\rightarrow$ {\tt doSaslHandshake()} $\rightarrow$ {\tt readSaslMessage()} $\rightarrow$ {\tt vintPrefixed} $\rightarrow$ {\tt read()}.
% ``{\color{red}-}'' means deleted code and 
``{\color{red}+}'' means added code, representing the patch transformed from TFix$^+$'s instrumented binary code. 
% ``{\protect\bluearrowsolid}'' represents the function call flows.
% ``{\protect\grayarrowdenselydotted}'' represents the data dependency flow.
}
\label{fig:Mapreduce-5066}
\end{figure}


==> lstStyle.tex <==
\makeatletter
\newenvironment{btHighlight}[1][]
{\begingroup\tikzset{bt@Highlight@par/.style={#1}}\begin{lrbox}{\@tempboxa}}
{\end{lrbox}\bt@HL@box[bt@Highlight@par]{\@tempboxa}\endgroup}

\newcommand\btHL[1][]{%
  \begin{btHighlight}[#1]\bgroup\aftergroup\bt@HL@endenv%
}
\def\bt@HL@endenv{%
  \end{btHighlight}%   
  \egroup
}
\newcommand{\bt@HL@box}[2][]{%
  \tikz[#1]{%
    \pgfpathrectangle{\pgfpoint{1pt}{0pt}}{\pgfpoint{\wd #2}{\ht #2}}%
    \pgfusepath{use as bounding box}%
    \node[anchor=base west, fill=orange!30,outer sep=0pt,inner xsep=1pt, inner ysep=0pt, rounded corners=3pt, minimum height=\ht\strutbox+1pt,#1]{\raisebox{1pt}{\strut}\strut\usebox{#2}};
  }%
}
\makeatother

\definecolor{javared}{rgb}{0.6,0,0} % for strings
\definecolor{javagreen}{rgb}{0.25,0.5,0.35} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc
\definecolor{bostonuniversityred}{rgb}{0.8, 0.0, 0.0}

%Define the style of lstlisting
% \lstdefinestyle{baseC}{
%   language=C,
%   tabsize=1,
%   breaklines=true,
%   basicstyle=\scriptsize\ttfamily\color{black},
%   showstringspaces=false,
%   moredelim=**[is][\color{red}]{@RED@}{@RED@},
%   moredelim=**[is][\color{bostonuniversityred}\textbf]{@DRED@}{@DRED@},
%   moredelim=**[is][\color{javadocblue}]{@BLUE@}{@BLUE@},
%   moredelim=**[is][{\btHL[fill=gray!40,thin]}]{@BG@}{@BG@},
%   keywordstyle=\color{javapurple}\bfseries,
%   stringstyle=\color{javadocblue},
%   commentstyle=\color{javagreen},
%   morecomment=[s][\color{bostonuniversityred}\textbf]{/*}{*/},
%   tabsize=4,
%   showspaces=false,
%   escapeinside={(*@}{@*)},
% }

\lstdefinestyle{baseJava}{
  language=Java,
  tabsize=1,
  breaklines=true,
  basicstyle=\scriptsize\ttfamily\color{black},
  showstringspaces=false,
  moredelim=**[is][\color{red}]{@RED@}{@RED@},
  moredelim=**[is][\color{bostonuniversityred}]{@DRED@}{@DRED@},
  moredelim=**[is][\color{javadocblue}]{@BLUE@}{@BLUE@},
  moredelim=**[is][\color{gray!50}]{@GRAY@}{@GRAY@},
  moredelim=**[is][{\btHL[fill=gray!30,thin]}]{@BG@}{@BG@},
  moredelim=**[is][{\btHL[fill=gray!30,thin]}]{@BLG@}{@BLG@},
  moredelim=**[is][\bfseries]{@BOLD@}{@BOLD@},
  keywordstyle=\color{javapurple}\bfseries,
  stringstyle=\color{javadocblue},
  commentstyle=\color{javagreen},
  morecomment=[s][\color{bostonuniversityred}]{/*}{*/},
  tabsize=4,
  showspaces=false,
  escapeinside={(*@}{@*)},
}

\newcommand{\tikzmark}[2]{%
     \tikz[overlay,remember picture] \node[text=black,
           inner sep=2pt] (#1) {#2};}
\newcommand{\VerticalShiftForArrows}{0.0em,2.75ex}
\newcommand{\VerticalShiftForBar}{0.0em,+2.0ex}
\newcommand{\VerticalShiftForOverArrows}{0.0em,+1.5ex}
\newcommand{\VerticalShiftForBelowArrows}{0.0em,-0.5ex}
\newcommand{\HorizonShiftForArrows}{0.0em,0.0ex}
\newcommand{\HorizonShiftForArrowsCustm}{0.0em,0.0ex}
\newcommand{\VerticalShiftForArrowsCustm}{0.0em,0.0ex}
\newcommand{\VerticalShiftForArrowss}{0.0em,2.75ex}
\newcommand{\VerticalShiftForArrowsss}{0.0em,2.75ex}
\newcommand{\VerticalShiftForArrowsCustms}{0.0em,0.0ex}
\newcommand{\HorizonShiftForArrowsCustms}{0.0em,0.0ex}
\newcommand{\VerticalShiftForArrowsC}{0.0em,0.0ex}
\newcommand{\VerticalShiftForArrowsCs}{0.0em,0.0ex}
\newcommand{\VerticalShiftForArrowsRtoLEnd}{0.0em,0.0ex}
\newcommand{\VerticalShiftForArrowsRtoRStart}{0.0em,0.0ex}
\newcommand{\Stub}{0.0em,-0.6ex}
\newcommand{\DrawOverBar}[3][]{
        \coordinate (top left)  at ($(#2)       +(\VerticalShiftForBar)$);
        \coordinate (start)     at ($(top left) +(\Stub)$);
        \coordinate (top right) at ($(#3)       +(\VerticalShiftForBar)$);
        \coordinate (end)       at ($(top right)+(\Stub)$);
        \draw [#1] (start) -- (top left) -- (top right) -- (end);
}
\newcommand{\DrawBelowOverArrows}[3][]{
        \coordinate (Start Below) at ($(#2Left)!0.5!(#2Right) + (\VerticalShiftForBelowArrows)$);
        \coordinate (End Above)   at ($(#3Left)!0.5!(#3Right) + (\VerticalShiftForOverArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Below) to (End Above);
}
\newcommand{\DrawBelowROverArrows}[3][]{
        \coordinate (Start Below) at ($(#2Right) + (\VerticalShiftForBelowArrows)$);
        \coordinate (End Above)   at ($(#3Left)!0.5!(#3Right) + (\VerticalShiftForOverArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Below) to (End Above);
}
\newcommand{\DrawBelowLeftOverLeftArrows}[3][]{
        \coordinate (Start Below) at ($(#2Left)!0.1!(#2Right) + (\VerticalShiftForBelowArrows)$);
        \coordinate (End Above)   at ($(#3Left)!0.1!(#3Right) + (\VerticalShiftForOverArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Below) to (End Above);
}
\newcommand{\DrawOverRightArrows}[3][]{
        \coordinate (Start Over) at ($(#2Left)!0.5!(#2Right) + (\VerticalShiftForOverArrows)$);
        \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Over) to (End Right);
}
\newcommand{\DrawOverBelowArrows}[3][]{
        \coordinate (Start Over) at ($(#2Left)!0.5!(#2Right) + (\VerticalShiftForOverArrows)$);
        \coordinate (End Below)   at ($(#3Left)!0.5!(#3Right) + (\VerticalShiftForBelowArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Over) to (End Below);
}
\newcommand{\DrawOverRBelowArrows}[3][]{
        \coordinate (Start Over) at ($(#2Right) + (\VerticalShiftForOverArrows)$);
        \coordinate (End Below)   at ($(#3Left)!0.5!(#3Right) + (\VerticalShiftForBelowArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Over) to (End Below);
}
\newcommand{\DrawOverRBelowLArrows}[3][]{
        \coordinate (Start Over) at ($(#2Right) + (\VerticalShiftForOverArrows)$);
        \coordinate (End Below)   at ($(#3Left) + (\VerticalShiftForBelowArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Over) to (End Below);
}
\newcommand{\DrawOverBelowLeftArrows}[3][]{
        \coordinate (Start Over) at ($(#2Left)!0.5!(#2Right) + (\VerticalShiftForOverArrows)$);
        \coordinate (End BelowLeft)   at ($(#3Left)!0.1!(#3Right) + (\VerticalShiftForBelowArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Over) to (End BelowLeft);
}
\newcommand{\DrawBelowBelowArrows}[3][]{
        \coordinate (Start Below) at ($(#2Left)!0.5!(#2Right) + (\VerticalShiftForBelowArrows)$);
        \coordinate (End Below)   at ($(#3Left)!0.5!(#3Right) + (\VerticalShiftForBelowArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Below) to (End Below);
}

\newcommand{\DrawArrows}[3][]{
    \coordinate (Start Mid) at ($(#2Left)!0.5!(#2Right) + (\VerticalShiftForArrows)$);
    \coordinate (End Mid)   at ($(#3Left)!0.5!(#3Right) + (\VerticalShiftForArrows)$);

    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Mid) to (End Mid);
}
\newcommand{\DrawBelowRightArrows}[3][]{
        \coordinate (Start Below) at ($(#2Left)!0.5!(#2Right) + (\VerticalShiftForBelowArrows)$);
        \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Below) to (End Right);
}
\newcommand{\DrawBelowRightArrowsCustm}[3][]{
        \coordinate (Start Below) at ($(#2Left)!0.5!(#2Right) + (\VerticalShiftForBelowArrows)$);
        \coordinate (End Right)   at ($(#3Right) $);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Below) to (End Right);
}
\newcommand{\DrawArrowsRight}[3][]{
    \coordinate (Start Right) at ($(#2Right) + (\VerticalShiftForArrows)$);
    \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrows)$);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Right) to (End Right);
}
\newcommand{\DrawArrowsRightHDFS}[3][]{
    \coordinate (Start Right) at ($(#2Right)$);
    \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrows)$);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Right) to (End Right);
}
\newcommand{\DrawArrowsRightHDFSNEW}[3][]{
    \coordinate (Start Right) at ($(#2Right) +(\VerticalShiftForArrowsCustm)$);
    \coordinate (End Right)   at ($(#3Right)$);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Right) to (End Right);
}
\newcommand{\DrawArrowsRightCustm}[3][]{
    \coordinate (Start Right) at ($(#2Right) + (\VerticalShiftForArrows)$);
%    \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrows) + (\HorizonShiftForArrows)$);
    \coordinate (top right) at ($(#3Right)       +(\VerticalShiftForArrowsss)$);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Right) to (top right);
}
\newcommand{\DrawArrowsRtoR}[3][]{
    \coordinate (Start Right) at ($(#2Right) + (\VerticalShiftForArrowsRtoRStart) $);
    \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrows) $);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Right) to (End Right);
}
\newcommand{\DrawArrowsRightCustmm}[3][]{
    \coordinate (Start Right) at ($(#2Right) + (\VerticalShiftForArrowss) $);
    \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrowss) $);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Right) to (End Right);
}
\newcommand{\DrawArrowsRtoL}[3][]{
    \coordinate (Start Right) at ($(#2Right) + (\VerticalShiftForArrows)$);
    \coordinate (End Left)   at ($(#3Left) + (\VerticalShiftForArrowsRtoLEnd)$);

    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Right) to (End Left);
}
\newcommand{\DrawArrowsRtoLCustm}[3][]{
    \coordinate (Start Right) at ($(#2Right) + (\VerticalShiftForArrows)+ (\HorizonShiftForArrowsCustm)$);
    \coordinate (End Left)   at ($(#3Left) + (\VerticalShiftForArrows) + (\VerticalShiftForArrowsCustm)$);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Right) to (End Left);
}
\newcommand{\DrawArrowsRtoLCustms}[3][]{
    \coordinate (Start Right) at ($(#2Right) + (\VerticalShiftForArrowsCustms) + (\VerticalShiftForArrowsC)$);
    \coordinate (End Left)   at ($(#3Left) +  (\VerticalShiftForArrowsCs)$);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Right) to (End Left);
}
\newcommand{\DrawRightOverArrows}[3][]{
        \coordinate (Start Right) at ($(#2Right) + (\VerticalShiftForArrows)$);
        \coordinate (End Above)   at ($(#3Left)!0.5!(#3Right) + (\VerticalShiftForOverArrows)$);
        \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Right) to (End Above);
}
\newcommand{\DrawArrowsLtoL}[3][]{
    \coordinate (Start Left) at ($(#2Left) + (\VerticalShiftForArrows)$);
    \coordinate (End Left)   at ($(#3Left) + (\VerticalShiftForArrows)$);

    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Left) to (End Left);
}
\newcommand{\DrawArrowsLtoLDouble}[3][]{
    \coordinate (Start Left) at ($(#2Left) + (\VerticalShiftForArrows)$);
    \coordinate (End Left)   at ($(#3Left) + (\VerticalShiftForArrows)$);

    \draw[line width=0.25mm, stealth-stealth, densely dotted, #1] (Start Left) to (End Left);
}
\newcommand{\DrawArrowsLtoR}[3][]{
    \coordinate (Start Left) at ($(#2Left) + (\VerticalShiftForArrows)$);
    \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrows)$);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Left) to (End Right);
}
\newcommand{\DrawArrowsLtoRCustm}[3][]{
    \coordinate (Start Left) at ($(#2Left) + (\HorizonShiftForArrowsCustm)$);
    \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrowsCustm)$);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Left) to (End Right);
}
\newcommand{\DrawArrowsLtoRCustms}[3][]{
    \coordinate (Start Left) at ($(#2Left) + (\VerticalShiftForArrowsCustms) + (\HorizonShiftForArrowsCustm)$);
    \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrows) + (\VerticalShiftForArrowsCustm)$);
    \draw[line width=0.25mm, -stealth, densely dotted, #1] (Start Left) to (End Right);
}
\newcommand{\DrawTwoArrowsRight}[3][]{
    \coordinate (Start Right) at ($(#2Right) + (\VerticalShiftForArrows)$);
    \coordinate (End Right)   at ($(#3Right) + (\VerticalShiftForArrows)$);

    \draw[line width=0.25mm, stealth-stealth, densely dotted, #1] (Start Right) to (End Right);
}

\newcommand{\grayarrowdenselydotted}{\raisebox{2pt}{\tikz{\draw[line width=0.25mm, -stealth, densely dotted, gray](0,0) -- (5mm,0);}}}
\newcommand{\bluearrowdashed}{\raisebox{2pt}{\tikz{\draw[line width=0.25mm, -stealth, dashed, azure](0,0) -- (5mm,0);}}}
\newcommand{\bluearrowlooselydashed}{\raisebox{2pt}{\tikz{\draw[line width=0.25mm, -stealth, loosely dashed, azure](0,0) -- (5mm,0);}}}
\newcommand{\bluearrowdenselydotted}{\raisebox{2pt}{\tikz{\draw[line width=0.25mm, -stealth, densely dotted, azure](0,0) -- (5mm,0);}}}
\newcommand{\bluearrowdashdotted}{\raisebox{2pt}{\tikz{\draw[line width=0.25mm, -stealth, dashdotted, azure](0,0) -- (5mm,0);}}}
\newcommand{\orangearrowdashed}{\raisebox{2pt}{\tikz{\draw[line width=0.25mm, -stealth, dashed, coral](0,0) -- (5mm,0);}}}
\newcommand{\orangearrowlooselydashed}{\raisebox{2pt}{\tikz{\draw[line width=0.25mm, -stealth, loosely dashed, coral](0,0) -- (5mm,0);}}}
\newcommand{\orangearrowdenselydotted}{\raisebox{2pt}{\tikz{\draw[line width=0.25mm, -stealth, densely dotted, coral](0,0) -- (5mm,0);}}}
\newcommand{\orangearrowdashdotted}{\raisebox{2pt}{\tikz{\draw[line width=0.25mm, -stealth, dashdotted, coral](0,0) -- (5mm,0);}}}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=0.5pt] (char) {#1};}}

\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{coral}{rgb}{1.0, 0.5, 0.31}

\definecolor{dkgreen}{rgb}{0,.6,0}
\definecolor{dkblue}{rgb}{0,0,.6}
\definecolor{dkyellow}{cmyk}{0,0,.8,.3}
\lstdefinestyle{baseHtml}{
  language=html,
  morekeywords={configuration, property, name, value, description},%
  tag=**[s]<>,%
  sensitive=f,%
  basicstyle      = \scriptsize\ttfamily\color{black},
  keywordstyle    = \color{javapurple}\bfseries,
  stringstyle     = \color{red},
  identifierstyle = \color{javadocblue},
  commentstyle    = \color{gray},
  emph            =[1]{html},
  emphstyle       =[1]\color{black},
  emph            =[2]{if,and,or,else},
  emphstyle       =[2]\color{dkyellow},
  moredelim=**[is][{\btHL[fill=gray!30,thin]}]{@BG@}{@BG@},
  moredelim=**[is][\color{javagreen}]{@GREEN@}{@GREEN@},
  morecomment=[s][\color{bostonuniversityred}\textbf]{/*}{*/},
  tabsize=4,
  showspaces=false,
  escapeinside={(*@}{@*)},
}

==> overhead.tex <==
\subsection{Overhead}

\begin{table}[]
\centering
\caption{The runtime overhead of TFix.}
\label{overhead}
\scriptsize
\setlength{\tabcolsep}{5mm}{
\begin{tabular}{|c|c|c|}
\hline
\textbf{System}   & \textbf{Workload}    & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}CPU Overhead\end{tabular}}}  \\ \hline\hline
Hadoop          & Word count & $0.29 \pm 0.023\%$                                \\ \hline
HDFS            & Word count & $0.44 \pm 0.050\%$                          \\ \hline
MapReduce       & Word count & $0.33  \pm 0.012\%$                           \\ \hline
Yarn      & Word count &    $0.38  \pm   0.025\%$                      \\ \hline
HBase          & YCSB & $0.41      \pm 0.024\%$                    \\ \hline
\end{tabular}}
\end{table}

\begin{comment}
\begin{table}[]
\centering
\caption{The runtime overhead of TFix.}
\label{overhead}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{System}   & \textbf{Workload}    & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Average CPU \\ Overhead\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Standard \\ Deviation of \\ CPU Overhead\end{tabular}}} \\ \hline\hline
Hadoop          & Word count & 0.29\%     & 0.023\%                                \\ \hline
HDFS            & Word count & 0.44\%     & 0.050\%                          \\ \hline
MapReduce       & Word count & 0.33\%     & 0.012\%                           \\ \hline
\textcolor{red}{Yarn}       & Word count &    0.38\%  &     0.025\%                      \\ \hline
HBase          & YCSB & 0.41\%            & 0.024\%                    \\ \hline
\end{tabular}
\end{table}
\end{comment}

In this subsection, we discuss the runtime overhead of TFix. 
TFix's runtime overhead comes from system call tracing, function call tracing and environment monitoring. Kernel level system call tracing only incurs less than 1\% overhead to the system~\cite{desnoyers2006lttng}. %The function call tracing, i.e., the Dapper tracing, is not always running for all the functions, which makes the overhead negligible.
Environment monitoring is cheap and the overhead is negligible~\cite{dean2011ubl}.
TFix enables function call tracing (the Dapper tracing) only on a small number of functions which are related to timeout configuration, network connection, and synchronization. We run the workloads on each system with and without tracing. We use the typical benchmarks for all server systems and impose the same types of workloads that trigger the tested timeout bugs. 
%TFix's function tracing module, i.e., Dapper framework, adopts an adaptive sampling strategy to reduce overhead. %If the system has a high workload, Dapper traces function calls at a higher frequency. Otherwise, Dapper traces %function calls at a lower frequency. 
We measure the tracing overhead and list the results in Table~\ref{overhead}. We observe that the overhead of TFix in terms of additional CPU load is less than 1\%, which makes it practical to apply TFix in real-world production systems.

==> prediction.tex <==
\begin{table*}[!t]
\centering
\caption{The prediction accuracy of TFix.}
\label{prediction}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Bug ID\end{tabular}} & \textbf{Bug Type} & \textbf{\begin{tabular}[c]{@{}c@{}}Under Estimation \\ Error\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Over Estimation \\ Error\end{tabular}} & \textbf{Standard Deviation} \\ \hline\hline
Hadoop-9106                                                                         &   too large timeout                                                                         &    0                            & 10.87\% &        1.35\%                                                                \\ \hline
Hadoop-11252 (v2.6.4)                                                                        &   too large timeout                                                                         &            0                   &  49.66\% &  7.11\%                                                                         \\ \hline
Hadoop-10695                                                                        &   too large timeout                                                                         &                                &   &                                                                         \\ \hline
HDFS-4301                                                                                       & too small timeout                                                                     & 0                                                                                                         & 14.3\% &    6.87\%                                                                  \\ \hline
HDFS-10223                                                                                       & too large timeout                                                                     &                                                                                                          &  &                                                                     \\ \hline
HDFS-9887                                                                                      & too small timeout                                                                     &                                     &  &                                                                     \\ \hline
MapReduce-6263                                                                                  &     too small timeout                                                                        &  1.06\%                                                                                                                & 0.12\% &  0.63\%                                                                     \\ \hline
MapReduce-4089                                                                         &   too large timeout                                                                        &    0                      &  7.94\% &  2.63\%                                                                       \\ \hline
Yarn-1630                                                                         &   too large timeout                                                                        &     2.68\%                     &   0.23\% & 1.71\%                                                                       \\ \hline
HBase-15645                                                                         &   too large timeout                                                                         &                          &   &                                                                       \\ \hline
HBase-17341                                                                         &   too large timeout                                                                         &          0                &  59.44\% &  4.30\%                                                                        \\ \hline
\end{tabular}
\end{table*}


\begin{comment}
Hadoop-9106                                                                         &   too large timeout                                                                         &    --                            & 4.43\% &                                                                        \\ \hline
HBase-17341                                                                         &   too large timeout                                                                         &    --                      &   &                                                                       \\ \hline
MapReduce-4089                                                                         &   too large timeout                                                                        &    --                      &   &                                                                       \\ \hline


\begin{tabular}[c]{@{}c@{}}replication.source\\ .maxretriesmultiplier\end{tabular}              & too small timeout                                                                            & 0                                                                                                                 & %28.3\% 
&                                                                      \\ \hline
mapreduce.task.timeout                                                                         &   too small timeout                                                                         &   0                                                                                                            &  2.16\% &                                                                      \\ \hline
\end{comment}


==> variableResult.tex <==
\begin{table}[!t]
\centering
\caption{The localized misused timeout variable.}
\label{variable_result}
\scriptsize
\begin{tabular}{|c|c|}
\hline
\textbf{Bug ID}       & \textbf{\begin{tabular}[c]{@{}c@{}}The Localized Misused \\ Timeout Variable\end{tabular}} \\ \hline\hline
Hadoop-9106           &  ipc.client.connect.timeout          \\ \hline
Hadoop-11252 (v2.6.4) &  ipc.client.rpc-timeout.ms       \\ \hline
Hadoop-10695 &    hadoop.security.kms.client.timeout    \\ \hline
HDFS-4301             &  dfs.image.transfer.timeout         \\ \hline
HDFS-10223            &  dfs.client.socket-timeout        \\ \hline
HDFS-9887            &   dfs.webhdfs.socket.connect-timeout      \\ \hline
MapReduce-6263        &  \begin{tabular}[c]{@{}c@{}}yarn.app.mapreduce.am \\.hard-kill-timeout-ms\end{tabular}         \\ \hline
MapReduce-4089        &  mapreduce.task.timeout       \\ \hline
Yarn-1630 (v2.3.0)      &   \begin{tabular}[c]{@{}c@{}}yarn.client.application-client-protocol \\.poll-timeout-ms \end{tabular}     \\ \hline
HBase-15645           &  hbase.client.operation.timeout         \\ \hline
HBase-17341           &  replication.source.maxretriesmultiplier          \\ \hline                                                                                                                                          
\end{tabular}
\end{table}
